Discrepancy Minimization in Input-Sparsity Time

A recent work by [Larsen, SODA 2023] introduced a faster combinatorial alternative to Bansal's SDP algorithm for finding a coloring $x \in \{-1, 1\}^n$ that approximately minimizes the discrepancy $\mathrm{disc}(A, x) := | A x |_{\infty}$ of a real-valued $m \times n$ matrix $A$. Larsen's algorithm runs in $\widetilde{O}(mn^2)$ time compared to Bansal's $\widetilde{O}(mn^{4.5})$-time algorithm, with a slightly weaker logarithmic approximation ratio in terms of the hereditary discrepancy of $A$ [Bansal, FOCS 2010]. We present a combinatorial $\widetilde{O}(\mathrm{nnz}(A) + n^3)$-time algorithm with the same approximation guarantee as Larsen's, optimal for tall matrices where $m = \mathrm{poly}(n)$. Using a more intricate analysis and fast matrix multiplication, we further achieve a runtime of $\widetilde{O}(\mathrm{nnz}(A) + n^{2.53})$, breaking the cubic barrier for square matrices and surpassing the limitations of linear-programming approaches [Eldan and Singh, RS&A 2018]. Our algorithm relies on two key ideas: (i) a new sketching technique for finding a projection matrix with a short $\ell_2$-basis using implicit leverage-score sampling, and (ii) a data structure for efficiently implementing the iterative Edge-Walk partial-coloring algorithm [Lovett and Meka, SICOMP 2015], and using an alternative analysis to enable ''lazy'' batch updates with low-rank corrections. Our results nearly close the computational gap between real-valued and binary matrices, for which input-sparsity time coloring was recently obtained by [Jain, Sah and Sawhney, SODA 2023].

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}


==> hard.tex <==
\section{Hardness}

\subsection{Hardness from Previous Work}\label{sec:lower_hardness}

We define a well-known hinted Mv problem from previous work \cite{bns19}.
\begin{definition}[Hinted Mv \cite{bns19}]\label{def:hintedMv}
    Let the computations be performed over the boolean semi-ring and let $m = n^\tau$, $0 < \tau \leq 1$. The hinted $Mv$ problem consists of the following phases:
    \begin{enumerate}
        \item Input two $n \times n$ matrices $M$ and $V$ \label{phase1}
        \item Input an $n\times n$ matrix $P$ with at most $n^\tau$ non-zero entries \label{phase2}
        \item Input a single index $i \in [n]$ \label{phase3}
        \begin{itemize}
            \item We need to answer $M P V_{*,i_t}$
            \item Here $V_{*,i_t} \in \R^n$ is the $i_t$-th column of matrix $V$
        \end{itemize}  
    \end{enumerate}
\end{definition}

We give the hinted Mv conjecture.
\begin{conjecture}[Hinted Mv conjecture \cite{bns19}]
\label{con:hintedMv}
    For every constant $0 < \tau \leq 1$ no algorithm for the hinted Mv problem (Definition~\ref{def:hintedMv}) can simultaneously satisfy
    \begin{itemize}
    \item polynomial time in phase \ref{phase1}
    \item $O (n^{\omega(1,1, \tau)-\epsilon} )$ time complexity in phase \ref{phase2} and
    \item $O (n^{1+\tau-\epsilon} )$ in phase \ref{phase3}
    \end{itemize}
    for some constant $\epsilon>0$.
\end{conjecture}


\subsection{Three phase version}
Inspired by \cite{bns19}, we define a three phase version.

\begin{definition}%[\Zhao{I write a definition}]
The  projection matrix vector multiplication $\mathsf{PMV}(n)$ consists of the following phases
\begin{enumerate}
    \item Input an $n \times n$ matrix $A$ 
    \item Input an $n \times n$ matrix $W$
    \item Input sequence of indices $\{i_1, \cdots, i_n \} \subset [n]$. We define $S_{t}:= \{ i_1, \cdots, i_t \}$
    \begin{itemize}
        \item Here $i_{t+1} \in [n]$ is only given after answering $\sum_{j \in S_{t+1} } w_j w_j^\top A_{*,i_{t+1}}$
        \item Here $w_j $ is $j$-th column of $W$, and $A_{*,i}$ is the $i$-th column of $A$
    \end{itemize}
\end{enumerate}
\end{definition}

\begin{definition}[Our setting] 
The projection matrix vector multiplication $\mathsf{PMV}(n)$ consists of the following phases
\begin{enumerate}
    \item Input an $n \times n$ matrix $A$ and a set $W_0 = \{w_1, w_2, \dots, w_\ell\} \subseteq \R^{n}$; 
    \item Input an $n \times n$ identity matrix $I_n \in \R^{n\times n}$;
    \item Input sequence of indices $\{i_1, \cdots, i_n \} \subset [n]$. %We define $S_{t}:= \{ i_1, \cdots, i_t \}$
    \begin{itemize}
        \item $w = (I - \sum_{w_j \in W_t} w_j w_j^\top)e_{i_{t+1}}$. $W_{t+1} \gets W_t \cup \{w\}$. 
        \item Here $e_{t+1} \in [n]$ is only given after answering $\sum_{w_j \in W_{t} } w_j w_j^\top A_{*,i_{t}}$
        \item Here $A_{*,i}$ is the $i$-th column of $A$. 
    \end{itemize}
\end{enumerate}
\end{definition}

\begin{remark}
    The output of our algorithm consists of the following two parts: 
    \begin{align*}
        A_{*,i_{t+1}} - \sum_{w_j \in W_{t+1}} w_j w_j^\top A_{*,i_{t+1}}.
    \end{align*}
    The first term is fixed. In this section we care about the second term. 
\end{remark}

==> omv.tex <==
\section{OMV with some known or not known Knowledge}

\begin{algorithm}[!ht]\caption{Data Structure }\label{alg:maintain_datastructure}
\begin{algorithmic}[1]
\State {\bf data structure} \textsc{OptimalMaintain} \Comment{Theorem~\ref{thm:omv_prior}}
\State {\bf members}
\State \hspace{4mm} $V \in \R^{n \times n}$
\State \hspace{4mm} $A \in \R^{n \times n}$ \Comment{Given matrix }
\State \hspace{4mm} $Q \in \R^{n \times n}$ \Comment{It is initialized by $Q  \gets {\bf 0}^{n \times n}$}
\State \hspace{4mm} $B \in \R^{n \times n}$ \Comment{We store the output}
\State \hspace{4mm} $\mathrm{prev}[n]$
\State {\bf end members}
\State 
\Procedure{Init}{$A$}
    \State $A\gets A$
    \State $V \gets 0^{n \times n}$ 
    \State $Q \gets 0^{n \times n}$
\EndProcedure
\State 
\Procedure{Update}{$w_i \in \R^{n}$, $i \in [n]$} \Comment{Lemma~\ref{lem:maintain_data_update_correct}, Lemma~\ref{lem:maintain_data_update_time}}
      \State $\Delta_i = 2^{ \lfloor \log (N/i) \rfloor}$  
        \State $\tau_{i,1} = [ \max\{i - \Delta_i + 1 , 1\} , i]$
        \State $\tau_{i,2} = [i, i + \Delta_i + 1] $
        
        \State $V_{i,*} \gets w_i^\top$ 
        
        \State $\wt{Q}_{*,\tau_{i,2}} \gets Q_{*,\tau_{i,2}} + ( V_{\tau_{i,1},*} )^\top {\bf 1}_{ \tau_{i,1} } V_{\tau_{i,1},*} A_{ *, \tau_{i,2} } $
        \State $B_{*,i} \gets  \wt{Q}_{*,i} $ 
        \State $Q \gets \wt{Q}$ 
\EndProcedure
\Procedure{Query}{$ i \in [n] $} \Comment{Lemma~\ref{lem:maintain_data_query_time}, Lemma~\ref{lem:maintain_data_query_correct}}
    \State \Return $B_{*,i}$
\EndProcedure
\State {\bf end data structure}
\end{algorithmic}
\end{algorithm}

\subsection{Main result}

\begin{theorem}
Given a matrix $A \in \R^{n \times n}$, there is a data that uses $O(n^2)$ space and supports the following operations
\begin{itemize}
    \item \textsc{Init}$(A,W \in \R^{n \times n})$. It takes $n^{2}$ time.
    %\item \textsc{Update}$(i \in [n],w_i \in \R^n)$. It takes $n^{\omega-1}$ amortized time.
    \item \textsc{Query}$(i)$. It outputs a length-$n$ vector that is equal to $(\sum_{j=1}^i w_j w_j^\top ) A_{*,i}$. It takes $n^{\omega-1}$ amortized time. Let $A_{*,i} \in \R^{n}$ denote the $i$-th column of matrix $A \in \R^{n \times n}$
\end{itemize}
Every time, we increase $i$ by $1$ when we call query function.
\end{theorem}

\begin{theorem}\label{thm:omv_prior}
Given a matrix $A \in \R^{n \times n}$, there is a data that uses $O(n^2)$ space and supports the following operations
\begin{itemize}
    \item \textsc{Init}$(A \in \R^{n \times n})$. It takes $n^{2}$ time.
    \item \textsc{Update}$(i \in [n],w_i \in \R^n)$. It takes $n^{\omega-1}$ amortized time.
    \item \textsc{Query}. It outputs a length-$n$ vector that is equal to $(\sum_{j=1}^i w_j w_j^\top ) A_{*,i}$. It takes $n^{\omega-1}$ amortized time. Let $A_{*,i} \in \R^{n}$ denote the $i$-th column of matrix $A \in \R^{n \times n}$
\end{itemize}
We alternative run one update and one query.
\end{theorem}

\begin{theorem}
Given a matrix $A \in \R^{n \times n}$, and a matrix $W \in \R^{n \times n}$, there is a data structure that uses $O(n^2)$ space and supports the following operations
\begin{itemize}
    \item \textsc{Init}$(A \in \R^{n \times n}, W \in \R^{n \times n})$. It takes $n^{\omega}$ time.
    \item \textsc{Update}$(i \in [n])$
    \item \textsc{Query}$(i \in [n])$ It outputs a length-$n$ vector that is equal to $(\sum_{j=1}^i w_j w_j^\top ) A_{*,i}$. It takes $n^{\omega-1}$ amortized time. Let $A_{*,i} \in \R^{n}$ denote the $i$-th column of matrix $A \in \R^{n \times n}$
\end{itemize}
Let $\{i_1, \cdots, i_n \} \subseteq [n]$. We alternatively run $\textsc{Update}(i_t)$ and $\textsc{Query}(i_t)$
\end{theorem}

\subsection{Three phase version}
Inspired by \cite{bns19}, we define a three phase version.

\begin{definition}[\Zhao{I write a definition}]
The amortized projection matrix vector multiplication $\mathsf{APMV}(n)$ consists of the following phases
\begin{enumerate}
    \item Input an $n \times n$ matrix $A$ 
    \item Input an $n \times n$ matrix $W$
    \item Input sequence of indices $\{i_1, \cdots, i_n \} \subset [n]$. We define $S_{t}:= \{ i_1, \cdots, i_t \}$
    \begin{itemize}
        \item Here $i_{t+1} \in [n]$ is only given after answering $\sum_{j \in S_{t+1} } w_j w_j^\top A_{*,i_{t+1}}$
        \item Here $w_j $ is $j$-th column of $W$, and $A_{*,i}$ is the $i$-th column of $A$
    \end{itemize}
\end{enumerate}
\end{definition}

\begin{definition}[Our setting \Yichuan{I changed above a little}]
The amortized projection matrix vector multiplication $\mathsf{APMV}(n)$ consists of the following phases
\begin{enumerate}
    \item Input an $n \times n$ matrix $A$; 
    \item Input an $n \times n$ matrix $W$;
    \item Input sequence of indices $\{i_1, \cdots, i_n \} \subset [n]$. We define $S_{t}:= \{ i_1, \cdots, i_t \}$
    \begin{itemize}
        \item Here $i_{t+1} \in [n]$ is only given after answering $(\sum_{j \in S_{0} } w_j w_j^\top + \sum_{j \in S_{t+1} } w_j w_j^\top) A_{*,i_{t+1}}$
        \item Here $w_j $ is $j$-th column of $W$, and $A_{*,i}$ is the $i$-th column of $A$, the $S_0 \subset[n]$ denotes the original projection matrx. 
    \end{itemize}
\end{enumerate}
\Yichuan{The output of our algorithm consists of three parts: 
\begin{align*}
    A_{*,i_{t+1}} - (\sum_{j \in S_{0} } w_j w_j^\top + \sum_{j \in S_{t+1} } w_j w_j^\top) A_{*,i_{t+1}}.
\end{align*}
}
\end{definition}

\subsection{Correctness}

\begin{lemma}[Correctness of Algorithm \ref{alg:maintain_datastructure} \textsc{Update}]\label{lem:maintain_data_update_correct}
When enter $\textsc{Update}$, assuming the following condition hold
\begin{itemize}
    \item Let $l$ denote smallest index in $\tau_{i,1}$ set, for each $t \in \tau_{i,2}$, we have $Q_{*,t} = \sum_{t=1}^{l-1} w_t w_t^\top A_{*,t} $
\end{itemize}
 Then, after we call $\textsc{Update}(w_i,i)$, the following holds
\begin{itemize}
    \item for all $t \leq i-1$, $ \wt{Q}_{*,t}$ are not changed at all
    \item $\wt{Q}_{*,i} = \sum_{j=1}^i w_j w_j^\top A_{*,i} $
    \item for $t \in \tau_{i,2}$,  $\wt{Q}_{*,t} = \sum_{j=1}^i w_j w_j^\top A_{*,t} $
\end{itemize}

\end{lemma}


\begin{proof}

{\bf Part 1.}

For each update, 
$\wt{Q}_{*,\tau_{i,2}} = Q_{*,\tau_{i,2}} + ( V_{\tau_{i,1},*} )^\top {\bf 1}_{ \tau_{i,1} } V_{\tau_{i,1},*} A_{ *, \tau_{i,2} } $ and $\tau_{i,2} = [i, i + \Delta_i + 1]$.

As $\tau_{i,2}$ begin from $i$, for all $t\leq i -1$, $\wt{Q}_{*,t}$ are not changed at all.
Hence, we complete the proof.



{\bf Part 2 and Part 3.}
???
% Next, we use induction to prove Part 2 and Part 3.

% For the base case, we have $\Delta_1 = N, \tau_{i,1} = \{1\}, \tau_{i,2} = [1,N+2]$.

% Then, we have
% $\wt{Q}_{*,[1,N]} = Q_{*,[1,N]} + ( V_{1,*} )^\top  V_{1,*} A_{ *, [1,N] } $
 

% \Zhao{To write a proof}
 
    
\end{proof}

\begin{lemma}[Correctness of Algorithm \ref{alg:maintain_datastructure} \textsc{Query}]\label{lem:maintain_data_query_correct}
    Let matrix $V \in \R^{ d\times n}$ be initialized by $V^0$. 
    
    Let $\mathsf{G} \in \R^{ n \times n}$ denote an input matrix.
    
    For each $i \in [n]$, we first call the function $\textsc{Update}(w_i,i)$ to update $V, Q$ and $G$. Then, we call the function $\textsc{Query}(i).$

    Function $\textsc{Query}(i)$ returns 
    \begin{align*}
    G_{*,i} =  (V_0^\top V_0 +\sum_{j=1}^i w_j w_j^\top ) \mathsf{G}_{*,i}
    \end{align*}
for each $i\in [n]$.
\end{lemma}


\begin{proof}
\begin{align*}
.
\end{align*}
    
\end{proof}

\subsection{Running Time}

\begin{lemma}[Running time of Algorithm \ref{alg:maintain_datastructure} \textsc{Update}]\label{lem:maintain_data_update_time}
    Let matrix $V \in \R^{ d\times n}$ be initialized by $V^0$. 
    
    Let $\mathsf{G} \in \R^{ n \times n}$ denote an input matrix.

    Let $\omega$ denote the current matrix multiplication exponent.
    
    For each $i \in [n]$, we  call the function $\textsc{Update}(w_i,i)$ to update $V, Q$ and $G$.

   It takes
\begin{align*}
    O(n^\omega)
\end{align*} time.
\end{lemma}

\begin{proof}
    Let $n_i = \max\{ | \tau_{i,1} | , | \tau_{i,2} | \}$.

Then we have
\begin{align*}
    n_i \leq & ~ \Delta_i + 1 \\
    \leq & ~ 2 \Delta_i \\
    \leq & ~ 2^{\log(N/i)} 
\end{align*}
where the second step follows from $\Delta_i \geq 1$.
%where $c > 2$ is some sufficiently large constant. \Tianyi{where we use this $c$?}


%\begin{itemize}
 %   \item 
    
    Computing $\mathsf{G}_{*,i} - ( {G}_{*,i} + Q_{*,i} )$ takes $O(n)$ time as we only compute the $i$-th column.
   % \item 

Let $c = 0.1$ denote a constant.
   
    The running time of computing $\mathsf{G}_{*,i} - ( {G}_{*,i} + Q_{*,i} )$ is


\begin{align*}
    \sum_{i=1}^N \Tmat(n, n_i ,n_i)
    = O(n^{\omega}) 
\end{align*}
where we use Lemma~\ref{lem:Tmat_n_n_i_n_i}

 
Hence, the total running time is $O(n^\omega)$.
\end{proof}


 

\begin{lemma}[Running time of Algorithm \ref{alg:maintain_datastructure} \textsc{Query}]\label{lem:maintain_data_query_time}
    Let matrix $V \in \R^{ d\times n}$ be initialized by $V^0$. 
    
    Let $\mathsf{G} \in \R^{ n \times n}$ denote an input matrix.

    Let $\omega$ denote the current matrix multiplication exponent.
    
    For each $i \in [n]$, we  call the function $\textsc{Query}(i)$ to get $G_{*,i}$.

   It takes
\begin{align*}
    O(n)
\end{align*} time.
\end{lemma}
\begin{proof}
    We only query for the $i$ column of $G$ so it takes $O(n)$ time.
\end{proof}


\iffalse
\begin{algorithm}[!ht]\caption{ \Zhao{Tianyi,  Ideally, I want to combine this algorithm with our dynamic attention problem.} }\label{alg:optimal_maintain}
\begin{algorithmic}[1]
\Procedure{OptimalMaintain}{$V \in \R^{d \times n}, \mathsf{G} \in \R^{n \times N}, b \in \{0,1\}^{n \times N}$}
    \State Let $d = n/4$. Let $N= \Theta(n)$ 
    \State $\sigma \gets {\bf 0}^N$
    \State $\wt{G} \gets (V^0)^\top V^0 \mathsf{G}$
    \Comment{$\wt{G} \in \R^{n \times N}, V^0 \in \R^{d \times n}$, this takes $n^{\omega}$ time}
    \State $Q \gets {\bf 0}^{n \times N}$
    \For{$i = 1 \to N$}
        \State $\Delta_i = 2^{ \lfloor \log (N/i) \rfloor}$ %\Comment{$\Delta_i = 2^{ \lfloor \log (N) - i \rfloor}$ }
        \State $\tau_{i,1} = [ \max\{i - \Delta_i + 1 , 1\} , i]$
        \State $\tau_{i,2} = [i, i + \Delta_i + 1] $
        \State We receive some online vector $w_i \in \R^n$ %black-box based on current $V$ and $b$
        \State $V^{i} \gets \begin{bmatrix} V^{i-1} \\ w_i^\top \end{bmatrix} \in \R^{(d+i) \times n}$ 
        \State $g_i \gets \mathsf{G}_{*,i} - ( \wt{G}_{*,i} + Q_{*,i} )$ \Comment{This is the vector we need to return}
        \State $Q_{*,\tau_{i,2}} \gets Q_{*,\tau_{i,2}} +  \underbrace{ (V^i_{\tau_{i,1},*} )^\top }_{n \times \Delta_i} \underbrace{ {\bf 1}_{ \tau_{i,1} } }_{\Delta_i \times \Delta_i} \underbrace{ V^i_{\tau_{i,1},*} }_{ \Delta_i \times n } \underbrace{ \mathsf{G}_{ *, \tau_{i,2} } }_{n \times \Delta_{i} } $
    \EndFor 
    \State \Return $g_1, \cdots, g_N$ \Comment{$g_i = ( ( V^i )^\top V^i \mathsf{G} )_{*,i}$ or $g_i = ( (I - ( V^i )^\top V^i ) \cdot \mathsf{G} )_{*,i}$}
\EndProcedure 
\end{algorithmic}
\end{algorithm}
\fi





